Style-Aware Normalized Loss for Improving Arbitrary Style Transfer

Neural Style Transfer (NST) has quickly evolved from single-style to infinite-style models, also known as Arbitrary Style Transfer (AST). Although appealing results have been widely reported in literature, our empirical studies on four well-known AST approaches (GoogleMagenta, AdaIN, LinearTransfer, and SANet) show that more than 50% of the time, AST stylized images are not acceptable to human users, typically due to under- or over-stylization. We systematically study the cause of this imbalanced style transferability (IST) and propose a simple yet effective solution to mitigate this issue. Our studies show that the IST issue is related to the conventional AST style loss, and reveal that the root cause is the equal weightage of training samples irrespective of the properties of their corresponding style images, which biases the model towards certain styles. Through investigation of the theoretical bounds of the AST style loss, we propose a new loss that largely overcomes IST. Theoretical analysis and experimental results validate the effectiveness of our loss, with over 80% relative improvement in style deception rate and 98% relatively higher preference in human evaluation.

==> archive/1_introduction.tex <==
\section{Introduction}

Style transfer refers to a procedure of changing the visual appearance of an image with a different given style while preserving the content. In Arbitrary Style Transfer(AST), the style image is given dynamically during runtime. Gatys\cite{} first proposed Neural Style Transfer(NST) which leverages the powerful Convolutional Neural Network in style transfer. Following works\cite{} adopt a feed-forward network to replace the slow optimization process in \cite{}, greatly boosting the speed of style transfer. 

Apart from several non-parametric style transfer works\cite{} which do not require style loss, most of style loss can be divided into three types, 1) Gram-based\cite{}, 2) discriminator-based\cite{} and 3) patch-swap-based\cite{}. Among them, discriminator-based method did not come out until recent years\cite{} while patch-swap-based method has a long history yet draws less attention. Plenty of works has been accomplished with Gram-based style loss\cite{}. 

Gram-based loss measures the difference between the Gram Matrices of two images' deep features. The deep features $\mathcal{F}(I) \in \mathbb{R}^{H \times W \times C}$ of an image $I$ is obtained by a pre-trained deep neural network. $H, W, C$ represent the height, width and feature dimension respectively. Afterwards, Gram Matrix is computed by tensor product of a reshaped deep feature $\mathcal{G}(\mathcal{F}(I)) = \mathcal{F}(I)^\intercal \cdot \mathcal{F}(I) \in \mathbb{R}^{C \times C}, where \, \mathcal{F}(I) \in \mathbb{R}^{(H \times W) \times C}$ is a reshaped feature. Style loss between two images is the mean-squared-error between their Gram Matrices $\mathcal{L}(I_i, I_j) = \frac{1}{C\times C}\left \| \mathcal{G}(\mathcal{F}(I_i)) - \mathcal{G}(\mathcal{F}(I_j)) \right \|^2$.

Total style loss is computed with deep features from a group of layers $L$ of deep neural network and then combined in order to capture both local and global style patterns. 

\begin{align}
    \mathcal{L}^l(I_i, I_j) &= \frac{1}{C^l\times C^l}\left \| \mathcal{G}(\mathcal{F}^l(I_i)) - \mathcal{G}(\mathcal{F}^l(I_j)) \right \|^2 \\
    \mathcal{L}^l(I_i, I_j) &= \sum_{l \in L} w_l \times \mathcal{L}^l(I_i, I_j)
\end{align}
$w_l$ is the style weight of layer $l$, which is usually set to same value\cite{} for all layers.

While effective, the Gram-based style loss does not always reflect the quality of style transfer. Fig.~\ref{fig.loss_histogram} shows the histogram of style losses of 2,000 random samples generated with AST model by \cite{}. Two images on the left has very small loss while style pattern are not transferred properly. On the contrary, right two images shows higher quality transferred image yet have large loss. We believe this counter-intuitive observation reveals a defect of Gram-based loss -- \textbf{style imbalance}.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/classic_loss_histogram.png}
    \includegraphics[width=\linewidth]{figures/normed_loss_histogram.png}
    \caption{(a) Loss distribution of classic Gram-based style losses of 2,000 random samples generated with four different methods \cite{}. Smaller loss does not guarantee better style transfer (left two images) while high quality transferred image can have large style loss (right two images). (b) Loss distribution of style balanced loss on 2,000 samples, . Content images are from ImageNet\cite{} and style images are from DTD\cite{}. Zoom in for better view.}
    \label{fig.loss_histogram}
\end{figure*}

We made following contributions in this paper. 1) We discover the defect of using conventional Gram-based style loss in the AST. 2) We conduct comprehensive studies to understand the root of the defect. 3) We proposed a style agnostic loss by using style-aware normalization to solve the style imbalance problem in current Gram-based AST. 4) Both qualitative and quantitative results show that the proposed method solves the imbalance problem among style images as well as style of different scales.

==> archive/2_related_works.tex <==
\section{Related Works}
\subsection{Neural Style Transfer}
Single style transfer, multi style transfer, arbitrary transfer.


==> archive/3_motivation.tex <==
\section{Motivation}\label{sec.3_motivation}
Given the style imbalance problem we observe from Fig.~\ref{fig.loss_histogram}, a natural question is: Is our observation generalizable? To verify how reliable the observation is, we conduct a human evaluation on 2,000 images used in Fig.~\ref{fig.loss_histogram}. Content and style images are randomly sampled from ImageNet\cite{} and Describable Texture Dataset(DTD)\cite{} respectively.

We find 5 volunteers and split 2,000 images evenly into 5 folds. Each volunteer is assigned to 400 images and is asked to score image by choosing one score from 1, 0 or -1 according to bad, moderate or good style transfer quality. Since this work only studies style loss, volunteers only need to score according to how good style has been transferred regardless of the fidelity of content. 

Criteria for scoring is as followed: Bad -- if a sample fails to transfer either color or texture. Moderate -- both color and texture are transferred but with recognizable distortion. Good -- both color and texture are transferred very well.

We compute the correlation between style loss and human scores. Ideally, the correlation score is close to 1 (i.e. the larger the loss, the worse the human score). 

\begin{table}[!h]
    \centering
    \small
    \begin{tabular}{c|ccccc}
        \hline
        Data & \multicolumn{5}{c}{VGG16 layer @ Block $x$ ReLU $y$ (b$x$\_r$y$)} \\ \cline{2-6}
        split & b1\_r2 & b2\_r2 & b3\_r3 & b4\_r4 & Total loss \\ \hline
        1 & -0.166 & -0.153 & -0.186 & -0.114 & -0.167  \\
        2 & -0.163 & -0.141 & -0.139 & -0.074 & -0.150  \\
        3 & -0.184 & -0.161 & -0.147 & -0.177 & -0.163  \\
        4 & -0.194 & -0.147 & -0.127 & 0.006 & -0.138  \\
        5 & -0.214 & -0.224 & -0.192 & -0.070 & -0.219  \\
        Overall & -0.168 & -0.148 & -0.114 & -0.059 & -0.136
    \end{tabular}
    \caption{Pearson Correlation between classic gram-based style loss and human score}
    \label{tab.classic_loss_human_coor}
\end{table}

\begin{table}[!h]
    \centering
    \small
    \begin{tabular}{c|ccccc}
        \hline
        Data & \multicolumn{5}{c}{VGG16 layer @ Block $x$ ReLU $y$ (b$x$\_r$y$)} \\ \cline{2-6}
        split & b1\_r2 & b2\_r2 & b3\_r3 & b4\_r4 & Total loss \\ \hline
        1 & -0.086 & 0.095 & 0.188 & 0.121 & 0.152  \\
        2 & 0.002 & 0.001 & 0.098 & 0.122 & 0.124  \\
        3 & -0.087 & 0.106 & 0.217 & 0.217 & 0.228  \\
        4 & -0.067 & -0.089 & 0.053 & 0.210 & 0.149  \\
        5 & -0.141 & -0.118 & 0.112 & 0.208 & 0.171  \\
        Overall & -0.083 & -0.030 & 0.108 & 0.176 & 0.153
    \end{tabular}
    \caption{Pearson Correlation between style balanced loss and human score}
    \label{tab.normed_loss_human_coor}
\end{table}

\textbf{A counterintuitive result} Contrary to expectations under ideal circumstances, results in Table.~\ref{tab.loss_human_coor} show a weak negative correlation between style loss and human scores. i.e. samples with higher loss have better transfer quality in general. It raises an important question. \textbf{What is the determining factor for style loss? Transfer quality or style image?}

To understand the root cause behind such counterintuitive observation, we conduct a comprehensive analysis in next section and find that the conventional Gram-based style loss is largely affected by the style instead of the quality of style transfer. Afterwards, we come up with a style-aware normalization to calibrate style loss so that the determining factors for loss is the transfer quality rather than style itself.


%  & \multicolumn{5}{c|}{Split} & Overall \\ \hline
%         Pearson & 1 & 2 & 3 & 4 & 5 & - \\
%         Correlation & a & b & c & d & e & f




\begin{comment}






In this section, we focus on finding what is wrong in the AST loss function and how to fix it. To simplify discussion, we focus on the style loss terms in the classic NST loss.

In particular, as pointed later in the section, it is not the classic NST loss function is wrong, but how it is used in AST task is wrong. More precisely, most AST approaches naturally extend the classic NST loss which is originally designed for a single style image and a single content image to the entire batch as shown in Eq.~\eqref{eq.ast_loss}, where $\loss_{\textrm{NST}}$ is defined in Eq.~\eqref{eq.nst_loss} and $B$ is the batch size.

\begin{equation}\label{eq.ast_loss}
\loss_{\textrm{AST}} = {1\over B}\sum_{k\in\{1,\cdots, B\}}\loss_{\textrm{NST}}(\im{S_k}, \im{T_k}) 
\end{equation}

Though Eq.~\eqref{eq.nst_loss} seems to be the standard way to compute the batch-wise loss from the sample-wise loss, it is inappropriate for the AST task. This is because unlike in other tasks, the sample loss in the AST task is not comparable to each other -- 


Given the style imbalance problem we observe from Fig.~\ref{fig.loss_histogram}, a natural question is: Is our observation generalizable? To verify how reliable the observation is, we conduct a human evaluation on 2,000 images used in Fig.~\ref{fig.loss_histogram}. Content and style images are randomly sampled from ImageNet\cite{} and Describable Texture Dataset(DTD)\cite{} respectively.

We find 5 volunteers and split 2,000 images evenly into 5 folds. Each volunteer is assigned to 400 images and is asked to score image by choosing one score from 1, 0 or -1 according to bad, moderate or good style transfer quality. Since this work only studies style loss, volunteers only need to score according to how good style has been transferred regardless of the fidelity of content. 

Criteria for scoring is as followed: Bad -- if a sample fails to transfer either color or texture. Moderate -- both color and texture are transferred but with recognizable distortion. Good -- both color and texture are transferred very well.

We compute the correlation between style loss and human scores. Ideally, the correlation score is close to 1 (i.e. the larger the loss, the worse the human score). 



\begin{table}[!h]
    \centering
    \small
    \begin{tabular}{c|ccccc}
        \hline
        Data & \multicolumn{5}{c}{VGG16 layer @ Block $x$ ReLU $y$ (b$x$\_r$y$)} \\ \cline{2-6}
        split & b1\_r2 & b2\_r2 & b3\_r3 & b4\_r4 & Total loss \\ \hline
        1 & -0.086 & 0.095 & 0.188 & 0.121 & 0.152  \\
        2 & 0.002 & 0.001 & 0.098 & 0.122 & 0.124  \\
        3 & -0.087 & 0.106 & 0.217 & 0.217 & 0.228  \\
        4 & -0.067 & -0.089 & 0.053 & 0.210 & 0.149  \\
        5 & -0.141 & -0.118 & 0.112 & 0.208 & 0.171  \\
        Overall & -0.083 & -0.030 & 0.108 & 0.176 & 0.153
    \end{tabular}
    \caption{Pearson Correlation between style balanced loss and human score}
    \label{tab.normed_loss_human_coor}
\end{table}

\textbf{A counterintuitive result} Contrary to expectations under ideal circumstances, results in Table.~\ref{tab.loss_human_coor} show a weak negative correlation between style loss and human scores. i.e. samples with higher loss have better transfer quality in general. It raises an important question. \textbf{What is the determining factor for style loss? Transfer quality or style image?}

To understand the root cause behind such counterintuitive observation, we conduct a comprehensive analysis in next section and find that the conventional Gram-based style loss is largely affected by the style instead of the quality of style transfer. Afterwards, we come up with a style-aware normalization to calibrate style loss so that the determining factors for loss is the transfer quality rather than style itself.


%  & \multicolumn{5}{c|}{Split} & Overall \\ \hline
%         Pearson & 1 & 2 & 3 & 4 & 5 & - \\
%         Correlation & a & b & c & d & e & f




\end{comment}

==> archive/4_method.tex <==
\section{Style Balanced Loss}


\subsection{Expectation of Style Loss} 
% \begin{itemize}
%     \item Derivation of $E[L(i, j)]$, i and j are two images
%     \item Use derived $E[L]$ to explain the reason of style imbalance is magnitude of gram matrix (euclidean norm of gram matrix)
%     \item A figure showing the histogram of original style loss of genuine and imposter distribution (on human labeling and PBN dataset), as well as a quantitative value of correlation between original style loss and magnitude of gram matrix
% \end{itemize}
To figure out the reason of imbalance in style transfer, we first compute the expectation of style loss between two arbitrary images. Without loss of generality, following derivation only considers style loss of a single layer and we omit term $\frac{1}{C \times C}$ since it is a constant. For simplicity, we use $\mathcal{G}_i$ to represent $\mathcal{G}(\mathcal{F}(I_i))$. 

Image $I_a$ can be seen as a random sample of the style $A$ it belongs to. Hence, its Magnitude of Gram Matrix $\left\|\mathcal{G}_a\right\|$\footnote{We use Euclidean Norm to represent Magnitude of Gram Matrix} follows $\left\|\mathcal{G}_a\right\| \sim P(\left\|\mathcal{G}_A\right\|)$, where $P(\left\|\mathcal{G}_A\right\|)$ is an unknown distribution of the Magnitude of Gram Matrix of style $A$. Even without knowing the actual distribution of $\left\|\mathcal{G}_A\right\|$, we can assume it has first and second order moments $\mu_A$ and $\sigma_A$ (i.e. $E[\left\|\mathcal{G}_A\right\|] = \mu_A$ and $Var[\left\|\mathcal{G}_A\right\|] = \sigma_A^2$).

\newtheorem{theorem}{Theorem}
\begin{theorem}
Given two image instances $a$ and $b$, which belongs to style $A$ and $B$, the expectation of style loss $E[\mathcal{L}(I_a, I_b)]$ is bounded by
\begin{equation}\label{eq.loss_bound}
    (\mu_A - \mu_B)^2 + \sigma_A^2 + \sigma_B^2 \leq E[\mathcal{L}(I_a, I_b)] \leq \mu_A^2 + \sigma_A^2 + \mu_B^2 + \sigma_B^2 
\end{equation}
\end{theorem}

\begin{proof}
\begin{align} \label{eq.expectation_of_loss}
    E[\mathcal{L}(I_a, I_b)] &= E[\left \| \mathcal{G}_a - \mathcal{G}_b \right \|^2] \\ \nonumber
    &= E[\left \| \mathcal{G}_a \right \|^2] + E[\left \| \mathcal{G}_b \right \|^2] - 2 \times E[\mathcal{G}_a \otimes \mathcal{G}_b] \\ \nonumber
    &= \underbrace{\mu_A^2 + \sigma_A^2 + \mu_B^2 + \sigma_B^2}_\textit{Term 1} - 2 \times \underbrace{E[\mathcal{G}_a \otimes \mathcal{G}_b]}_\textit{Term 2}
\end{align}
$\otimes$ is element-wise product between two matrices. \textit{Term 1} is because of $E[x^2] = Var[x] + E[x]^2$ for a random variable $x$. \textit{Term 2} in the Eq.~\ref{eq.expectation_of_loss} is bounded.
\begin{align}\label{eq.term2_upper_bound}
    E[(\mathcal{G}_a \otimes \mathcal{G}_b)] &= E[\sum_{k \in C\times C} \mathcal{G}_{a,k} \times \mathcal{G}_{b,k}] \\ \nonumber
    &\stackrel{\textcircled{\raisebox{-0.9pt}{1}}}{=} E[\mathcal{G}_{a,flatten}^\intercal \cdot \mathcal{G}_{b,flatten}] \\ \nonumber
    &\stackrel{\textcircled{\raisebox{-0.9pt}{2}}}{\leq} E[\left \| \mathcal{G}_a \right \| \left \| \mathcal{G}_b \right \|] \\ \nonumber
    &= \mu_A \mu_B
\end{align}
Step $\textcircled{\raisebox{-0.9pt}{1}}$ is by rewriting summation into a dot product. Step $\textcircled{\raisebox{-0.9pt}{2}}$ is because of Cauchy–Schwarz inequality. 

\begin{align}\label{eq.term2_lower_bound}
    E[(\mathcal{G}_a \otimes \mathcal{G}_b)] = E[\sum_{k \in C\times C} \mathcal{G}_{a,k} \times \mathcal{G}_{b,k}] \geq 0
\end{align}
because Gram Matrix is computed from features output by a ReLU layer, all values in the matrix are non-negative.

Replace \textit{Term 2} in Eq.~\eqref{eq.expectation_of_loss} with Eq.~\eqref{eq.term2_upper_bound},~\eqref{eq.term2_lower_bound}, the expectation of style loss is bounded by
\begin{equation}
    (\mu_A - \mu_B)^2 + \sigma_A^2 + \sigma_B^2 \leq E[\mathcal{L}(I_a, I_b)] \leq \mu_A^2 + \sigma_A^2 + \mu_B^2 + \sigma_B^2 \nonumber
\end{equation}

\end{proof}


As above mentioned, the actual distribution of $\left \| \mathcal{G}_{A/B} \right \|$ is unknown. A good empirical value of $\mu_A$ can be obtained with $\left \| \mathcal{G}_a \right \|$ since $E[\left \| \mathcal{G}_a \right \|] = \mu_A$. However, it is difficult to even have an approximation for $\sigma_A$. To get rid of variance, we derive a \textbf{variance free form of $E[\mathcal{L}(I_a, I_b)]$.} 

\begin{theorem}
Given two image instances $a$ and $b$, which belongs to style $A$ and $B$, the expectation of style loss $E[\mathcal{L}(I_a, I_b)]$ has relaxed bounds
\begin{equation}\label{eq.relaxed_loss_bound}
    (\mu_A - \mu_B)^2 \leq E[\mathcal{L}(I_a, I_b)] \leq k(\mu_A^2 + \mu_B^2)
\end{equation}
where $k > 0$ is a constant depending on loss model.
\end{theorem}

\begin{proof}
We do two relaxation on Eq.~\eqref{eq.loss_bound}.
\begin{equation}\label{eq.relax_left}
    E[\mathcal{L}(I_a, I_b)] \geq (\mu_A - \mu_B)^2
\end{equation}
which is easy to obtain since $\sigma_{A/B} \geq 0$. 

We use Bhatia–Davis inequality\cite{} $\sigma^2 \leq (M-\mu)(\mu-m)$ (where $M$ and $m$ are upper bound and lower bound of the random variable) to find the relaxed upper bound. Bhatia–Davis inequality requires the distribution of random variable is bounded which can be guaranteed in our case. 1) $\left \| \mathcal{G}_a \right \|$ has a lower bound $m=0$ since it is the Euclidean Norm of a real value matrix. 2) $\left \| \mathcal{G}_a \right \|$ has an upper bound since it is computed with a bounded input image and a fixed real value neural network by consecutive summations and multiplications. We denote this upper bound with $M$.


Therefore, there exists a constant $k>0$ such that for any style $S$, there is $k \mu_S \geq M$\footnote{We do not consider the trivial case when $\mu_S=0$}. The relaxed upper bound of $E[\mathcal{L}(I_a, I_b)]$ is:
\begin{align}
    \sigma_{A}^2 &\leq (M-\mu_A)(\mu_A-m) \\ \nonumber
    &\leq (k \mu_A - \mu_A)\mu_A \\ \nonumber
    &= (k-1)\mu_A^2 \\
    E[\mathcal{L}(I_a, I_b)] &\leq k(\mu_A^2 + \mu_B^2) \label{eq.relax_right}
\end{align}

Combining Eq.~\eqref{eq.relax_left} and~\eqref{eq.relax_right}, the variance free form of Eq.~\eqref{eq.loss_bound} is:
\begin{equation}
    (\mu_A - \mu_B)^2 \leq E[\mathcal{L}(I_a, I_b)] \leq k(\mu_A^2 + \mu_B^2) \nonumber
\end{equation}
\end{proof}

\subsection{Imbalance in Style Loss}
A reasonable subsequent conjecture from Eq.~\ref{eq.relaxed_loss_bound} will be -- For style that has larger moments($\mu_A$ and $\mu_B$), its style loss increases due to both lower bound and upper bound of the style loss are increased. To validate this conjecture, we leverage our human labeling and the Painter-by-numbers dataset.

On human labeling dataset, we treat style image and stylized image as $I_a$ and $I_b$. 

On Painter-by-numbers dataset, we randomly sampled 10,000 pairs of images for $I_a$ and $I_b$.

\textbf{Correlation of $\mathcal{L}(I_a, I_b)$ and Lower/Upper Bound}. We use $\left\|\mathcal{G}_{a}\right\|$, satisfying $E[\left\|\mathcal{G}_{a}\right\|]=\mu_A$, as an empirical approximation for $\mu_A$ and compute correlation of 1) $\mathcal{L}(I_a, I_b)$ and $(\left\|\mathcal{G}_{a}\right\| - \left\|\mathcal{G}_{b}\right\|)^2$; 2) $\mathcal{L}(I_a, I_b)$ and $\left\|\mathcal{G}_{a}\right\|^2 + \left\|\mathcal{G}_{b}\right\|^2$. 

% \begin{table}[!h]
%     \centering
%     \begin{tabular}{c|cccc}
%     \hline
%         Loss layer & b1\_r2 & b2\_r2 & b3\_r3 & b4\_r3 \\ \hline \hline
%         Human labeling & 0.782 & 0.791 & 0.844 & 0.965 \\
%         Painter-by-numbers  & 0.879 & 0.925 & 0.901 & 0.804 \\ \hline
%     \end{tabular}
%     \caption{Pearson Correlation of $\mathcal{L}(I_a, I_b)$ and $(\left\|\mathcal{G}_{a}\right\| - \left\|\mathcal{G}_{b}\right\|)^2$}
%     \label{tab.lower_bound_coor}
%     \vspace{1em}
%     \begin{tabular}{c|cccc}
%     \hline
%         Loss layer & b1\_r2 & b2\_r2 & b3\_r3 & b4\_r3 \\ \hline \hline
%         Human labeling & 0.517 & 0.895 & 0.779 & 0.838 \\
%         Painter-by-numbers  & 0.912 & 0.754 & 0.824 & 0.918 \\ \hline
%     \end{tabular}
%     \caption{Pearson Correlation of $\mathcal{L}(I_a, I_b)$ and $\left\|\mathcal{G}_{a}\right\|^2 + \left\|\mathcal{G}_{b}\right\|^2$}
%     \label{tab.upper_bound_coor}
% \end{table}

Fig.~\ref{fig.corr_before_norm} shows the Pearson Correlation with features from different layers of a pre-trained VGG16 network\cite{}. The strong correlation of style loss and lower/upper bound confirms the fact that style images have a huge impact on style loss, which is the root cause of negative correlation observed in Sec.~\ref{sec.3_motivation}.

\subsection{Style-Aware Normalization}
The imbalanced style loss, as a result, causes imbalanced optimization during training. Styles that yield larger losses get more change to be optimized while those with smaller losses are less optimized. 

Under certain circumstance, the lower bound of one pair of images' style loss can be higher than the upper bound of another pair of images' loss (e.g. when pair $(a, b)$ and $(c, d)$ satisfy $(\mu_A - \mu_B)^2 \geq k(\mu_C^2 + \mu_D^2)$). We propose to normalize style loss according to its style inputs, i.e. a style-aware normalization, by dividing $\mu_A^2 + \mu_B^2$.

\begin{equation}
    \widehat{\mathcal{L}}(I_a, I_b) = \frac{\mathcal{L}(I_a, I_b)}{\mu_A^2 + \mu_B^2}
\end{equation}

The expectation of normalized loss $\widehat{\mathcal{L}}(I_a, I_b)$ will have lower bound $1 - \frac{2\mu_A\mu_B}{\mu_A^2 + \mu_B^2}$, which has range $[0, 1]$, and upper bound equals to $k$ for an arbitrary pair of images. In practice, as mentioned above, we use $\left\|\mathcal{G}_{a}\right\|$ as a substitute for $\mu_{A}$ due to lack of actual value of $\mu_{A}$.

\subsection{Effect of Style-Aware Normalization on Real Data}
% Show the histogram of style loss on human labeling and PBN dataset
% \begin{itemize}
%     \item Original style loss
%     \item Normalized style loss (sum)
% \end{itemize}

\textbf{Reduce correlation between style loss and style.} 


\begin{figure}[t]
    \centering
    \scriptsize{Human labeling}\par
    \includegraphics[width=\linewidth]{figures/correlation/corr_human_before_norm_diff.png}
    \includegraphics[width=\linewidth]{figures/correlation/corr_human_before_norm_sum.png}
    \scriptsize{Painter-by-numbers}\par
    \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_before_norm_diff.png}
    \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_before_norm_sum.png}
    \caption{Correlation between classic Gram-based loss and styles}
    \label{fig.corr_before_norm}

\end{figure}

\begin{figure}[t]
    \centering
    \scriptsize{Human labeling}\par
    \includegraphics[width=\linewidth]{figures/correlation/corr_human_after_norm_diff.png}
    \includegraphics[width=\linewidth]{figures/correlation/corr_human_after_norm_sum.png}
    \scriptsize{Painter-by-numbers}\par
    \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_after_norm_diff.png}
    \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_after_norm_sum.png}
    \caption{Correlation between style balanced loss and styles}
    \label{fig.corr_after_norm}
\end{figure}

\textbf{Align loss with human expectation.}
To better understand how style-aware normalization changes the distribution of loss, we leverage the Painter-by-numbers to plot the Genuine Imposter Curve. 



% \newcommand{\rulesep}{\unskip\ \vrule\ }
% \begin{figure*}
%     \centering
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \scriptsize{Human labeling}\par
%         \includegraphics[width=\linewidth]{figures/correlation/corr_human_before_norm_diff.png}
%         \includegraphics[width=\linewidth]{figures/correlation/corr_human_before_norm_sum.png}
%         \scriptsize{Painter-by-numbers}\par
%         \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_before_norm_diff.png}
%         \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_before_norm_sum.png}
%         \caption{Correlation between classic Gram-based loss and styles}
%         \label{fig:sub1}
%     \end{subfigure}
%     \rulesep
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \scriptsize{Human labeling}\par
%         \includegraphics[width=\linewidth]{figures/correlation/corr_human_after_norm_diff.png}
%         \includegraphics[width=\linewidth]{figures/correlation/corr_human_after_norm_sum.png}
%         \scriptsize{Painter-by-numbers}\par
%         \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_after_norm_diff.png}
%         \includegraphics[width=\linewidth]{figures/correlation/corr_pbn_after_norm_sum.png}
%         \caption{Correlation between normalized loss and styles}
%         \label{fig:sub2}
%     \end{subfigure}
%     \caption{Figures on the left show that style loss is strongly correlated to the style it takes as input. }
% \end{figure*}

==> archive/5_experiment.tex <==
\section{Experiments}
The proposed style balanced loss is method agnostic for all gram-matrix based approaches. To show the wide generality of our method, we conduct experiments on four different approaches\cite{} which has open access code. 

\textbf{AdaIN}\cite{} introduce a fast-feed forward neural network for arbitrary style transfer. They use a pretrained VGG16\cite{} model to extract image features and match the statistic of the content features with those of the style features by using an adaptive instance normalization layer. 

\textbf{Magenta}\cite{} use a pretrained InceptionNet\cite{} to extract style image feature and use it as a prior for the conditional instance normalization to align content feature and style feature. 

\textbf{SANET}\cite{} introduce a style-attentional network to maintain local and global pattern in the same time. An identity loss and multi-level feature aggregation are used to preserve content structure as well as style pattern. 

\textbf{LinearTransfer}\cite{} extracts content and style image features with a pretrained VGG\cite{} model. A linear transformation matrix is calculated by composing content and style features and used to transform content features to aligns the mean and covariance of the target style. 

We compare the result of using classic gram based loss and style balanced loss. 

\subsection{Qualitative Evaluation}

\begin{figure}[!h]
    \centering
    \scriptsize{Content \qquad\qquad\;\;  Style \qquad\; Style Balance Loss \   Classic Gram Loss \ \ \ }\par
    \includegraphics[width=\linewidth]{figures/qualitative1.png}
    \includegraphics[width=\linewidth]{figures/qualitative2.png}
    \caption{Qualitative comparison between models trained with style balanced loss and classic gram-based loss. (TODO NEED MORE SAMPLES)}
    \label{fig.qualitative_compare_to_baseline}
\end{figure}

\subsection{Quantitative Evaluation}
\begin{itemize}
    \item Loss distribution on testing subset?
    % \item Loss curve during training?
    % \item Deception rate comparison with previous arbitrary style transfer
    % \item User study?
\end{itemize}

\textbf{Training Speed}
Using style balanced loss accelerates the training. Fig.~\ref{fig.training_loss} shows the training loss curve of four approaches with classic gram based loss and style balanced loss. Since the loss model and loss layers used for loss computation is not same for different approaches. We change all loss model to VGG16 and loss layers to b1\_r2,b2\_r2,b3\_r3,b4\_r3 in order to plot all curves in same figure. Similar result can also be obtained with VGG19 and different loss layers, please refer to Appendix~\ref{} for details. We can see that after applying style balanced loss, balabala...

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/training_loss.png}
    \caption{Training style loss of our \textcolor{SkyBlue}{style balanced loss} and \textcolor{Salmon}{classic style loss}. Both loss curves are plotted with original style loss metric.}
    \label{fig.training_loss}
\end{figure}

\textbf{User Study}
We generate 200 image pairs for each style transfer approach\cite{} above mentioned. Every image pair has two transferred images which use same content and style image. One transferred image is generated by model trained with classic Gram-based loss and one by model trained with style balanced loss. Content images are sampled from ImageNet\cite{} and style images are from PBN\cite{} and DTD\cite{}, each with 50 images. Every user is shown with 20 images and is asked to vote for the one he/she prefers. We use Amazon Mechanical Turk to collect ??? votes from ??? users. The result is shown in Fig.~\ref{}. 



\textbf{Deception Rate}
Deception Rate is an evaluation method introduced by Sanakoyeu\cite{} for quantitatively measuring style transfer quality. The method computes the success rate of stylized images deceiving an artist classification model. 
In our experiment, we generate 3,000 stylized images with different Arbitrary Style Transfer models. Content images are randomly sampled from ImageNet and style images are collected from 30 artists with most works on Painter-by-numbers dataset(PBN). 

We use the released code of the winning solution\footnote{https://github.com/inejc/painters} for Painter-by-numbers challenge to compute deception rate. The model returns a 2048 dimension feature for each image. We computed image features of paintings from 30 artists with most works in PBN. A transferred image from artist $X$'s painting is considered successfully deceiving the model if its nearest neighbour in feature space comes from same artist $X$. 

From table~\ref{tab.deception_rate} we can see that after using style balanced loss, the deception rate has been largely increased...

\begin{table}[!h]
    \centering
    \small
    \begin{tabular}{c|cc}
    \hline
        \multicolumn{2}{c}{Method} &  Deception Rate (in \%)\\ \hline
        Classic   & AdaIN\cite{} &  \\
        Style& Magenta\cite{} &  \\ 
        Loss & SANET\cite{} &  \\ 
        & LinearTf\cite{} &  \\ \hline
        Style & AdaIN\cite{} & \\
        Balanced  & Magenta\cite{} & \\
        Loss & SANET\cite{} & \\
        & LinearTf\cite{} & \\ \hline
    \end{tabular}
    \caption{Deception rate of different method}
    \label{tab.deception_rate}
\end{table}
